Imaging local diffusion in microstructures using NV-based pulsed field gradient NMR

Understanding diffusion in microstructures plays a crucial role in many scientific fields, including neuroscience, cancer or energy research. While magnetic resonance (MR) methods are the gold standard for diffusion measurements, spatial encoding in MR imaging has limitations. Here, we introduce nitrogen-vacancy (NV) center based nuclear magnetic resonance (NMR) spectroscopy as a powerful tool to probe diffusion with an optical readouts. We have developed an experimental scheme combining pulsed gradient spin echo (PGSE) with optically detected NV-NMR spectroscopy, which allows for the local quantification of molecular diffusion and flow within microscopic sample volumes. We demonstrate correlated optical imaging with spatially resolved PGSE NV-NMR experiments probing anisotropic water diffusion within a model microstructure. Our optically detected PGSE NV-NMR technique opens up prospects for extending the current capabilities of investigating diffusion processes with the future potential of probing single cells, tissue microstructures, or ion mobility in thin film materials for battery applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
